Multi-layer Representation Learning for Medical Concepts

Learning efficient representations for concepts has been proven to be an important basis for many applications such as machine translation or document classification. Proper representations of medical concepts such as diagnosis, medication, procedure codes and visits will have broad applications in healthcare analytics. However, in Electronic Health Records (EHR) the visit sequences of patients include multiple concepts (diagnosis, procedure, and medication codes) per visit. This structure provides two types of relational information, namely sequential order of visits and co-occurrence of the codes within each visit. In this work, we propose Med2Vec, which not only learns distributed representations for both medical codes and visits from a large EHR dataset with over 3 million visits, but also allows us to interpret the learned representations confirmed positively by clinical experts. In the experiments, Med2Vec displays significant improvement in key medical applications compared to popular baselines such as Skip-gram, GloVe and stacked autoencoder, while providing clinically meaningful interpretation.

==> algorithm.tex <==
\begin{algorithm}[t]
\caption{Training \mname \label{alg:med2vec}} 
Initialize $\Wb_c, \Wb_h, \bb_c, \bb_h$ randomly\;
\For{$i=1$ to epoch} 
{
	\Repeat{Change of the Frobenius norm of $\Wb_c < \epsilon$}
    {
    	\ForEach{mini-batch of visit sequence} 
        {
            Evaluate the gradients\;
            Update $\Wb_c, \Wb_h, \bb_c, \bb_h$ using the gradients\;
            Project $\Wb_c$ onto $\Wb_c \geqslant 0$\;
            Evaluate the Frobenius norm of $\Wb_c$\;
        }
	}	
}
\end{algorithm}

==> cms_dataset.tex <==
\begin{table}[t]
\caption{Basic statistics of the CMS dataset.}
\label{tab:cms_stats}
\small
\vspace*{-2mm}
\centering
\begin{tabular}{l|r}
\hline
\# of patients & 831,210 \\ 
\# of visits & 5,464,950 \\
Avg. \# of visits per patient & 6.57 \\
\hline
\# of unique medical codes & 21,033 \\
- \# of unique diagnosis codes & 14,111 \\
- \# of unique procedure codes & 6,922 \\
\hline
Avg. \# of codes per visit & 3.19 \\
\hline
Max \# of codes per visit & 44 \\
\hline
(95\%, 99\%) percentile \# of codes per visit & (9, 13) \\
\hline
\end{tabular}
\vspace*{-2mm}
\end{table}

==> visit_label_stats.tex <==
\begin{table}[t]
\caption{Basic statistics of cRG levels and the number of specialties}
\label{tab:visit_label_stats}
\vspace{0.1in}
\centering
\begin{tabular}{l|c|c|c}
\hline
Label & Task & \# of classes & \# of visits \\ 
\hline
\scriptsize{CRG level} & \scriptsize{Logistic reg.} & 2 & 672,110 \\
%Charges & \scriptsize{Linear reg.} & N/A & 672,129 \\
\scriptsize{\# of Spc.} & \scriptsize{Linear reg.} & 20 & 672,110 \\
\hline
\end{tabular}
\vspace{-0.1in}
\end{table}

